Evaluating Language Models for Generating and Judging Programming Feedback

The emergence of large language models (LLMs) has transformed research and practice across a wide range of domains. Within the computing education research (CER) domain, LLMs have garnered significant attention, particularly in the context of learning programming. Much of the work on LLMs in CER, however, has focused on applying and evaluating proprietary models. In this article, we evaluate the efficiency of open-source LLMs in generating high-quality feedback for programming assignments and judging the quality of programming feedback, contrasting the results with proprietary models. Our evaluations on a dataset of students' submissions to introductory Python programming exercises suggest that state-of-the-art open-source LLMs are nearly on par with proprietary models in both generating and assessing programming feedback. Additionally, we demonstrate the efficiency of smaller LLMs in these tasks and highlight the wide range of LLMs accessible, even for free, to educators and practitioners.

==> data/table/tabular/judging.tex <==
\begin{tabular}{lllllllll}
\toprule
judge & EA & ES & EC & FA & FS & FC & AVGO & AVGS \\
\midrule
phi-3-mini & 0.70 (-0.04) & 0.29 (-0.16) & 0.81 (-0.03) & 0.70 (-0.06) & 0.34 (-0.21) & 0.81 (-0.03) & 0.56 (-0.12) & 0.44 (+0.13) \\
mistral & 0.67 (+0.08) & 0.07 (+0.20) & 0.78 (+0.02) & 0.66 (+0.08) & 0.08 (+0.19) & 0.76 (+0.06) & 0.44 (+0.12) & 0.47 (-0.03) \\
llama3.1-8b & 0.69 (+0.07) & 0.19 (+0.23) & 0.80 (+0.01) & 0.65 (+0.12) & 0.30 (+0.21) & 0.79 (+0.01) & 0.53 (+0.10) & 0.41 (+0.10) \\
ensemble & 0.70 (+0.07) & 0.09 (+0.10) & 0.81 (-0.01) & 0.68 (+0.06) & 0.17 (+0.06) & 0.80 (+0.01) & 0.48 (+0.06) & nan (+nan) \\
llama3.1-70b & 0.71 (-0.17) & 0.67 (+0.17) & 0.84 (-0.03) & 0.71 (-0.06) & 0.66 (+0.16) & 0.82 (-0.03) & 0.68 (+0.06) & 0.58 (+0.15) \\
gpt-3.5-turbo & 0.71 (-0.02) & 0.10 (+0.00) & 0.79 (+0.00) & 0.68 (-0.04) & 0.16 (-0.03) & 0.78 (+0.00) & 0.47 (-0.02) & 0.54 (+0.02) \\
gpt-4o-mini & 0.77 (+0.04) & 0.30 (-0.01) & 0.81 (+0.01) & 0.77 (+0.01) & 0.42 (-0.07) & 0.82 (+0.00) & 0.57 (+0.02) & 0.59 (+0.04) \\
gpt-4o & 0.74 (+0.02) & 0.78 (+0.02) & 0.81 (-0.03) & 0.70 (+0.05) & 0.75 (+0.06) & 0.82 (-0.03) & 0.70 (+0.01) & 0.68 (+0.12) \\
\bottomrule
\end{tabular}
